Ulam meets Turing: constructing quadratic maps with non-computable SRB measures

In 1946, S. Ulam invented Monte Carlo method, which has since become the standard numerical technique for making statistical predictions for long-term behaviour of dynamical systems. We show that this, or in fact any other numerical approach can fail for the simplest non-linear discrete dynamical systems given by the logistic maps $f_{a}(x)=ax(1-x)$ of the unit interval. We show that there exist computable real parameters $a\in (0,4)$ for which almost every orbit of $f_a$ has the same asymptotical statistical distribution in $[0,1]$, but this limiting distribution is not Turing computable.

==> preliminaries_measures.tex <==
% !TEX root = main.tex


\section{Preliminaries}





 
 \subsection*{Statistical simulations and computability of probability measures}
 
We give a very brief summary of relevant notions of Computability Theory and Computable Analysis. For a more in-depth
introduction, the reader is referred to e.g. \cite{BY-book}.
As is standard in Computer Science, we formalize the notion of
an algorithm as a {\it Turing Machine} \cite{Tur}.  
We will call a  function $f:\NN\to\NN$  \emph{computable} (or {\it recursive}), if there exists a Turing Machine  $\cM$ which, upon input $n$, outputs $f(n)$.
Extending algorithmic notions to functions of real numbers was pioneered by Banach and Mazur \cite{BM,Maz}, and
is now known under the name of {\it Computable Analysis}. 
Let us begin by giving the modern definition of the notion of computable real
number,  which goes back to the seminal paper of Turing \cite{Tur}. By identifying $\Q$ with $\N$ through some effective enumeration, we can assume algorithms can operate on $\Q$. Then a real number $x\in\RR$ is called \defin{computable} if there is an algorithm  $M$ which, upon input $n$, halts and outputs a rational number $q_n$ such that  $|q_n-x|<2^{-n}$.
Algebraic numbers or  the familiar constants such as $\pi$, $e$, or the Feigenbaum constant  are computable real numbers. However, the set of all computable real numbers $\RR_C$ is necessarily countable, as there are only countably many Turing Machines. 

We now define computability of functions over $[0,1]$.  Recall that for a continuous function $f\in C_{0}([0,1])$, a modulus of continuity consists of a function $\delta: \Q\cap(0,a)\to\Q\cap(0,a)$ such that $|f(x)-f(y)|\leq \epsilon$ whenever $|x-y|\leq \delta(\epsilon)$. A function $f:[0,1]\to[0,1]$ is \defin{computable} if it has a computable modulus of continuity and there is an algorithm which, provided with a rational number which is $\delta(\epsilon)$-close to $x$, outputs a rational number which is $\epsilon$-close to $f(x)$.  

Computability of probability measures, say over $[0,1]$ for instance, is defined by requiring the ability to compute the expected value of computable functions. 

\begin{defn}\label{1}Let $(f_{i})$ be any sequence of uniformly computable functions over $[0,1]$. A probability measure $\mu$ over $[0,1]$ is \defin{computable} if there exist a Turing Machine $M$ which on input $(i,\epsilon)$ (with $\epsilon \in \Q$) outputs a rational $M(i,\epsilon)$ satisfying
$$
|M(i,\epsilon) - \int f_{i}\,d\mu | < \epsilon.
$$
\end{defn}

We note that this definition it compatible with the notion of weak convergence (see Section \ref{stage}) of measures in the sense that a measure is computable if and only if it can be algorithmically approximated (in the weak topology) to an arbitrary degree of accuracy by measures supported on finitely many rational points and with rational weights.  
Moreover, this definition also models well the intuitive notion of statistical sampling in the sense that a measure $\mu$ is computable if and only if there is an algorithm to convert sequences sampled from the uniform distribution into sequences sampled with respect to $\mu$. 

In this paper, we will be interested in the computability properties of invariant measures of  quadratic maps of the form $ax(1-x)$, with $a\in \RR$. 
%As is standard in computing practice, we will assume that the algorithm can read the value of $a$ externally in order to compute $\mu$. More formally, let us denote $\cD_n\subset \RR$ the set of dyadic rational numbers with denominator $2^{-n}$. 
%We say that a function $\phi:\NN\to\QQ$ is an {\it oracle} for $a\in \RR$ if for every $m\in \NN$
%$$\phi(m)\in \cD_m\text{ and }d(\phi(m),a)<2^{-(m-1)}.$$
%We amend our definitions of computability of a probability measure $\mu$ by allowing {\it oracle Turing Machines} $M^\phi$ where $\phi$ is any function as above. 
%On each step of the algorithm, $M^\phi$ may read the value of $\phi(m)$ for an arbitrary $m\in\NN$.
%This approach, usually referred to as computability {\it relative to} $a$, allows us to separate the questions of computability of a parameter $a$ from that of the measure.

%We will use the following terminology. A compact set $K$ is \emph{lower computable} if there is a sequence $x_{i}\in K$ of uniformly computable points\footnote{A sequence $x_i$ is uniformly computable if there is a single algorithm which, upon input $(n,i)$ computes $x_i$ at precision $n$} which is dense in $K$. It is called \emph{upper-computable} if  its complement is a lower-computable open set\footnote{An open set is lower computable if it is the union of a computable sequence of rational intervals.}. It is not hard to see that a set $K$ is computable if and only if it is lower and upper computable. 


\subsection*{Invariant measures of quadratic polynomials and the statement of the main result.}
As before, we denote 
$$f_a(x)=ax(1-x).$$
For $a\in[0,4]$, this quadratic polynomial maps the interval $[0,1]$ to itself. We will view $f_a:[0,1]\to[0,1]$ as a discrete dynamical system, and will denote $f_a^n$ the $n$-th iterate of $f_a$. 

A measure $\mu$ is called \defin{physical} or {\it Sinai-Ruelle-Bowen (SRB)} if 
\begin{equation}\label{srb}
\frac{1}{n}\sum_{k=0}^{n-1}\delta_{f^{k}x} \to \mu 
\end{equation}
for a set of positive Lebesgue measure.  It is known that if a physical measure exists for a quadratic map $f_{a},\,\, a\in [0,4]$, then it is unique and (\ref{srb}) is satisfied for Lebesgue almost all $x\in [0,1]$. 



\bigskip
\noindent\textbf{Main Theorem.} \emph{
There exist computable parameters $a\in(0,4)$ for which the quadratic map $f_a(x)=ax(1-x)$ has a physical measure $\mu$ which is not computable. 
	}
\bigskip

\noindent
We note that in the version of this work which was presented at STOC-2020 \cite{RY-STOC}, we showed the existence of an uncountable set of parameters for which the physical measure exists but is not computable, yet the proof was not constructive. 




